Hidden Monotonicity: Explaining Deep Neural Networks via their DC Decomposition

It has been demonstrated in various contexts that monotonicity leads to better explainability in neural networks. However, not every function can be well approximated by a monotone neural network. We demonstrate that monotonicity can still be used in two ways to boost explainability. First, we use an adaptation of the decomposition of a trained ReLU network into two monotone and convex parts, thereby overcoming numerical obstacles from an inherent blowup of the weights in this procedure. Our proposed saliency methods - SplitCAM and SplitLRP - improve on state of the art results on both VGG16 and Resnet18 networks on ImageNet-S across all Quantus saliency metric categories. Second, we exhibit that training a model as the difference between two monotone neural networks results in a system with strong self-explainability properties.

==> latexmkrc <==
# Latexmk configuration for multibib support
# This tells latexmk to run bibtex on the appendix bibliography

# Add custom dependency for multibib 'app' bibliography
add_cus_dep('aux', 'bbl', 0, 'run_bibtex');

sub run_bibtex {
    system("bibtex \"$_[0]\"");
}

# Ensure these extensions are cleaned up
push @generated_exts, 'bbl', 'blg';


==> sections/multiplicative_networks.tex <==
\subsection{Multiplicative Networks} \label{subsec:polynomial_ops}

In this section we lay the theoretical foundation to split neural networks that contain non-additive network components as Gating, SE-Blocks or attention modules.
For these components we need to split the stream through matrix multiplication layers and Hadamard product layers.
Moreover, we need to approximate smooth functions (as Softmax and the Sigmoid function) by CPWL functions.

We prove a general Theorem in \cref{app:splitting_multiplicative_maxout_networks}, where we define the framework of so-called rank-$k$ Maxout Multiplication networks.
However, we want to state the Theorem here translated to a more application-focused language restricted to ReLU networks.
Recall that a posynomial is a polynomial with positive coefficients.
To state the Theorem, we generalize the notion of \emph{monotone} and \emph{input convex} to general neural networks containing linear, convolutional, maximum, matrix product and Hadamard product components in the natural way.

\begin{theorem} \label{thm:main_simplified}
    Any (residual) ReLU network $N$ containing linear, convolutional, maximum, matrix product and Hadamard product components can be split into two rank-$2$ monotone Maxout networks $N^+$ and $N^-$, that each calculate the maximum of a finite set of posynomials in the network input variables ($N = N^+ - N^-$).
    Furthermore, it can be split into two input-convex rank-$2$ monotone Maxout networks $\tilde{N}^+$ and $\tilde{N}^-$, that each calculate convex functions ($N = \tilde{N}^+ - \tilde{N}^-$).
\end{theorem}
